Granger Causal Interaction Skill Chains

Reinforcement Learning (RL) has demonstrated promising results in learning policies for complex tasks, but it often suffers from low sample efficiency and limited transferability. Hierarchical RL (HRL) methods aim to address the difficulty of learning long-horizon tasks by decomposing policies into skills, abstracting states, and reusing skills in new tasks. However, many HRL methods require some initial task success to discover useful skills, which paradoxically may be very unlikely without access to useful skills. On the other hand, reward-free HRL methods often need to learn far too many skills to achieve proper coverage in high-dimensional domains. In contrast, we introduce the Chain of Interaction Skills (COInS) algorithm, which focuses on controllability in factored domains to identify a small number of task-agnostic skills that still permit a high degree of control. COInS uses learned detectors to identify interactions between state factors and then trains a chain of skills to control each of these factors successively. We evaluate COInS on a robotic pushing task with obstacles -- a challenging domain where other RL and HRL methods fall short. We also demonstrate the transferability of skills learned by COInS, using variants of Breakout, a common RL benchmark, and show 2-3x improvement in both sample efficiency and final performance compared to standard RL baselines.

==> scratch.tex <==
Now that we can identify an interaction between two factors, we want to train a skill using existing skills controlling source factor(s) to interact with one of the target factors. This requires three design choices: which source factor to use, which target factor to connect it to, and how to learn control over the target factor. In this work, we use the last factor we learned skills over as the source factor, which constructs a chain. Future work can extend this to other controllable factors or even groups of factors to form a general hierarchy.
% For the source factor, we choose the factor we most recently learned skills over. Initially, this is the primitive actions, but as we learn more skills, this might be other factors like the paddle, the ball, etc. in Breakout. For the target factor, we choose an uncontrolled factor (one without corresponding skills) with the highest interaction score (Equation~\ref {hypothesis_test}). This iterative skill chaining is similar to that described in HyPE~\cite{chuck2020hypothesis}, and constructs a chain as illustred in Figure~\ref{main_figure}. These choices of source and target can be adapted in future work to form other structures from trees to DAGs or even cycles in the summary graph. Below, we describe how to train a parameterized skill to control that factor.

% \subsubsection{Object Option Chains}
% The Chain of Interaction Skills (COInS) algorithm defines each layer of the hierarchy by goal-based control of one of the factors. Each option $\omega_i$ corresponds to one factor, \textit{e.g.}, $\omega_\text{Paddle}$, or $\omega_\text{Gripper}$ with $\omega_1$ corresponding to primitive actions. COInS then discovers a sequence $\omega_{1}, \hdots \omega_{K}$ which describes a goal-based skill to control each factor in the hierarchy using the skills $\omega_{i-1}$ it has already learned. 
% Each skill is defined by a goal-based policy and termination condition where the action space of $\omega_i$ corresponds to the goal space of $\omega_{i-1}$, as described in the Background and illustrated in Figure~\ref{option_chain}. COInS iteratively builds up from $\omega_1$, connecting a new factor $i+1$ to $i$ at iteration $i$ of COInS.
\subsubsection{Determining Target Factor Control}
In order to determine which target factor to control, COInS evaluates $\text{Sc}_{I}(D,a,b)$ for all $b$, where $a$ indexes the last factored with learned control, and $b$ indexes a factor that COInS has not yet learned to control. COInS then selects as target factor the factor with the highest interaction score:
\begin{equation}
b = \argmin_b \text{Sc}_{I}(D,a,b)
\label{highestinteraction}
\end{equation}

However, just because one factor ($a$) can affect the dynamics of another ($b$) does not mean that every goal is reachable in a reasonable horizon. Certain features $\xv_b[k]$ of the target factor $\xv_b$ might be controllable, while others may not. For example in Breakout, the paddle affects the ball dynamics, but within one timestep of an interaction, the ball position cannot be directly controlled. Trying to control both the ball position and velocity simultaneously would result in many infeasible goals. To address this, COInS alters the goals by applying a control mask $\eta_b \in \{0,1\}^K$ where $K$ is the number of features in factor $\xv_b$.   

% While many goal-based RL methods rely on higher-level controllers to determine goals in the full state space, the high dimensionality of this space can often cause these methods to fail~\cite{levy2018hierarchical}. Instead, COInS uses partial control: Only learn to control interactions, and only learn to control the particular features of the target factor which can be controlled, denoted with a control mask $\eta$ which we define below.

% Instead, COInS focuses on two key insights: First, control happens at interactions. Second, not every feature of a factor can be controlled through an interaction. For example, only the velocity of the ball is controlled with the paddle at an interaction, not the position directly. To exploit this, factor goals are filtered by interactions and goals are masked with a control mask $\eta_b$.

% A state factor such as the state of the ball in breakout might contain several state features, like the ball's velocity and position. $\eta$ is a length $f$ (number of features) binary vector: $\{0,1\}^f$. $\eta[i]$ is the $i$-th feature of $\eta$. $\eta[i]=1$ for feature $i$ that can be controlled directly. 

To identify controllable features (1s in $\eta_b$), we use the following intuition: if the feature value differs significantly from the passive prediction after an interaction with the source factor, that suggests the source factor caused the change. This property can be evaluated over a dataset $D$ with $\mu(m^\text{pas}(\xb;\theta))$ as the mean of the passive prediction and $N_\text{int}$ as the number of interactions in the dataset:
\begin{equation}
\eta_b[i] = \begin{cases} 1 & \frac{1}{N_\text{int}}\sum_{\xa, \xb, \xb' \sim D}h(\xa, \xb, \xb';\theta,\psi) \left\|\xb'[i] - \mu(m^\text{pas}(\xb;\theta))\right\| > 1-\epsilon_\eta\\
0 & \text{otherwise},
\end{cases}
\label{eta_test}
\end{equation}
For examples of $\eta$-masks and post-interaction states, see Section~\ref{Experiments}. If the size of the \textit{unique masked post-interaction state set} $\mathcal C_b\coloneqq unique(\eta_b \mathcal \xvs_b)$ is sufficiently small, $|\mathcal C_b| < n_\text{disc}$, then we sample discretely.


